Mutiny! How does Kubernetes fail, and what can we do about it?

In this paper, we i) analyze and classify real-world failures of Kubernetes (the most popular container orchestration system), ii) develop a framework to perform a fault/error injection campaign targeting the data store preserving the cluster state, and iii) compare results of our fault/error injection experiments with real-world failures, showing that our fault/error injections can recreate many real-world failure patterns. The paper aims to address the lack of studies on systematic analyses of Kubernetes failures to date. Our results show that even a single fault/error (e.g., a bit-flip) in the data stored can propagate, causing cluster-wide failures (3% of injections), service networking issues (4%), and service under/overprovisioning (24%). Errors in the fields tracking dependencies between object caused 51% of such cluster-wide failures. We argue that controlled fault/error injection-based testing should be employed to proactively assess Kubernetes' resiliency and guide the design of failure mitigation strategies.

==> 8_failures.tex <==
\begin{table*}[]
\begin{tabular}{|l|l|l|l|}
\hline
Effect                                         & Problem                                       & Cause                                       & Solution \\ \hline
 Cluster outage                                 & Impossible to elect etcd leader               & Byzantine link failure between masters      &          \\ \hline
 Huge number of Pods created                    & ReplicaSet not recognized by Deployment & New scheduling feature                      &          \\ \hline
 Fail to fully deploy Service & Less Pod than expected                        & Buggy custom plugin  &          \\ \hline
 Fail to scale Service                          & Conflicting commands by the autoscaler        & Autoscaler implementation                   &          \\ \hline
 Cluster outage                                 & All master nodes drained                      & Human error                                 &          \\ \hline
 Cluster outage (almost)                       & Master node out of memory                     & Overload                                    &          \\ \hline
 Application slowdown x2                        & Throttling of applications                    & Worker node Linux scheduler                 &          \\ \hline
 Application OOM kill                           & CPU Throttling                                & Bad dimensioning and backpressure &          \\ \hline
 Application not spawning                       & Container images deleted                      & Buggy custom job                            &          \\ \hline
Application not spawning                       & Fail to pull images                     & Pull rate limiting/Misconfiguration                            &          \\ \hline
 Cluster outage                                 & Networking broken                             & Change in labeling between versions         &          \\ \hline
 Massive Service deletion                       & Error in template configuration               & Configuration error                         &          \\ \hline
 Connection failures towards outside         & Networking misconfiguration                   & Configuration error                         &          \\ \hline
 Event drop for Services                        & Partial DNS resolution outage                 & Stale conntrack     &          \\ \hline
 Slow Service deploy                        & Fail to schedule Pods                            & Virtual IP addresses exhaustion             &          \\ \hline
 Delay in Pod communication                     & DNS resolution failure                        & Linux networking race condition             &          \\ \hline
 Many Pods killed                                & Cluster overcrowded                           & Workload deployed as DaemonSet              &          \\ \hline
 Pod overcrowding                               & Pod startup resource usage triggers autoscale                    & Autoscaler algorithm                        &          \\ \hline
 Services shutdown                              & Pod not ready                                 & Failing sidecar container                   &          \\ \hline
 Worker node panic                              & Pods overcrowd worker node                    & Configuration error                         &          \\ \hline
 Custom Resources not updated                     & Status field not updated         & Policy change in K8s upgrade                         &          \\ \hline
 Cluster outage  & Master node resource exhaustion & Fail to retrieve huge amount of objects \\ \hline
Fail to reach Service  & Network manager unhealthy & Fail to retrieve huge amount of objects \\ \hline
Fail to reach Service  & DNS unhealthy & Out of memory/Misconfiguration \\ \hline
  Cannot schedule Pods   & No Worker Nodes, cannot join & Change of URL in rpm package \\ \hline
Cluster outage (almost)  & Apiserver intermittent failure and nodes deleted & Apiserver plugin hang during bootstrap \\ \hline
Intermittent 502 response from Service & Pod shutdown before Endpoint removal & Parallel processing, bad app programming \\ \hline
Cluster outage & State corrupted & Human error \\ \hline
Failing worker nodes & Kubelet error & Out of memory \\ \hline
Connection errors & DNS blackhole & Stale conntrack \\ \hline
Application scaled down & Removed replica number defaulted to one & Apiserver algorithm \\ \hline
Slow deployment of Services & Overfilled scheduling queue & Huge number of unschedulable Pods \\ \hline
\end{tabular}
\end{table*}
